Simulated Tempering Langevin Monte Carlo II: An Improved Proof using Soft Markov Chain Decomposition

A key task in Bayesian machine learning is sampling from distributions that are only specified up to a partition function (i.e., constant of proportionality). One prevalent example of this is sampling posteriors in parametric distributions, such as latent-variable generative models. However sampling (even very approximately) can be #P-hard. Classical results going back to Bakry and \'Emery (1985) on sampling focus on log-concave distributions, and show a natural Markov chain called Langevin diffusion mixes in polynomial time. However, all log-concave distributions are uni-modal, while in practice it is very common for the distribution of interest to have multiple modes. In this case, Langevin diffusion suffers from torpid mixing. We address this problem by combining Langevin diffusion with simulated tempering. The result is a Markov chain that mixes more rapidly by transitioning between different temperatures of the distribution. We analyze this Markov chain for a mixture of (strongly) log-concave distributions of the same shape. In particular, our technique applies to the canonical multi-modal distribution: a mixture of gaussians (of equal variance). Our algorithm efficiently samples from these distributions given only access to the gradient of the log-pdf. For the analysis, we introduce novel techniques for proving spectral gaps based on decomposing the action of the generator of the diffusion. Previous approaches rely on decomposing the state space as a partition of sets, while our approach can be thought of as decomposing the stationary measure as a mixture of distributions (a "soft partition"). Additional materials for the paper can be found at http://holdenlee.github.io/Simulated%20tempering%20Langevin%20Monte%20Carlo.html. The proof and results have been improved and generalized from the precursor at arXiv:1710.02736.

==> body.tex <==

\input{st}
\input{decomp}
%\input{gap.tex}
%\input{gap2}
\input{st-gaussians-new}
\input{discretization}
\input{main-proof}





==> gap.tex <==

\section{Markov chain decomposition theorems}
\label{sec:mcd}
\subsection{$\chi^2$ Gap-Product Theorem}

The main Markov chain decomposition theorem we use to prove Theorem~\ref{thm:main} is Theorem~\ref{thm:gap-prod-st}. As a warm-up, we first prove a simpler gap-product theorem, Theorem~\ref{thm:gap-prod}.

Note that Theorem~\ref{thm:gap-prod} is incomparable to the original by~\cite{madras2002markov}. In their theorem, they decompose $\Om$ into a partition, the projected chain is on the sets of the partition, and the transition probabilities are the probabilities of transitioning between the two sets. Here, we decompose into a sum of probability distributions instead (a soft partition), and the transition probabilities in the projected chain is determined by the $\chi^2$-distance between the distributions.
%TODO: there may be a way of generalizing both at the same time, by allowing the chi^2 distance to be one-way.

We state the theorem for continuous Markov chains; it works for discrete chains with the appropriate modifications.

\begin{thm}[$\chi^2$ Gap-Product Theorem]
\label{thm:gap-prod}
Let $M=(\Om, \sL)$ be a continuous-time Markov chain with stationary distribution $p$ and Dirichlet form $\sE(g,g)=-\an{g,\sL g}$. Suppose the following hold.
\begin{enumerate}
\item
There is a decomposition
\begin{align}
p\sL &= \sumo jm w_jp_j \sL_j\\
%\an{g, \sL g}_p &= \sumo jm w_j \an{g,\sL_j g}_{p_j}\\
p&= \sumo jm w_jp_j.
\end{align}
where $\sL_j$ is the generator for some Markov chain $M_j$ on $\Om$ with stationary distribution $p_{j}$.
\item
(Mixing for each $M_j$) The Dirichlet form $\sE_j(f,g) = -\an{f,\sL_j g}_{p_j}$ satisfies the Poincar\'e inequality
\begin{align}
\Var_{p_j}(g) &\le C \sE_j(g,g).
\end{align}
\item
(Mixing for projected chain) 
Define the $\chi^2$-projected chain $\ol M$ as the Markov chain on $[m]$ generated by $\ol{\sL}$, where $\ol{\sL}$ acts on $\ol g\in L^2([m])$ by
\begin{align}
\ol{\sL} \ol g(j) &= \sum_{1\le k\le m, k\ne j} [\ol g(k)-\ol g(j)]
\ol P(j,k)\\
%\rc{\chi^2(p_j||p_k)} \min\bc{\fc{w_k}{w_j}, 1}.
\text{where }
\ol P(j,k) &= \fc{w_k}{\max\{\chi^2(p_j||p_k)
, \chi^2(p_k||p_j)\}}
.
\end{align}
(I.e., the rate of diffusion from $j$ to $k$ is given by $\ol P(j,k)$.) %, which is the continuous version of Metropolis-Hastings sampling.)
Let $\ol p$ be the stationary distribution of $\ol M$.
Then $\ol M$ satisfies the Poincar\'e inequality
\begin{align}
\Var_{\ol p} (\ol g) & \le \ol C \ol{\sE}(g,g).
\end{align}
\end{enumerate}
Then $M$ satisfies the Poincar\'e inequality
\begin{align}
\Var_p(g) &\le C \pa{1+\fc{\ol C}2} \sE(g,g).
\end{align}
\end{thm}
\begin{proof}
First, note that the stationary distribution $\ol p$ of $\ol M$ is given by $\ol p(j) = w_j$, because $w_j\ol P(j,k) = w_k \ol P(k,j)$. (Note that the reaston $\ol P$ has a maximum of $\chi^2$ divergences in the denominator is to make this ``detailed balance'' condition hold.)

Given $g\in L^2(\Om)$, define $\ol g\in L^2([m])$ by $\ol g(j) = \EE_{p_j} g$. Then
\begin{align}
\Var_p(g) &=\sumo jm w_j \int (g-\E g)^2p_j\\
&=\sumo jm w_j \int (g-\EE_{p_j} g)^2 p_j
+ \sumo jm w_j (\EE_{p_j} g - \EE_p g)^2\\
&\le \sumo jm w_j \int (g-\EE_{p_j} g)^2 p_j + \sumo jm \ol p(j) (\ol g(j) - \EE_{\ol p}\ol g)^2\\
&\le C \sumo jm w_j \sE_{p_j}(g,g) + \Var_{\ol p}(\ol g)\\
&\le C \sE(g,g) + \ol C \ol \sE (\ol g, \ol g).
\label{eq:to-cont}
\end{align}
%where we used the fact that the stationary distribution of $\ol M$ is $\ol p$ given by $\ol p(j) = w_j$, because $w_j\ol P(j,k) = w_k \ol P(k,j)$. 
Now
\begin{align}
\ol \sE (\ol g, \ol g) &= \rc 2\sumo jm \sumo km (\ol g(j)-\ol g(k))^2 w_j \ol P(j,k) \\
&\le \rc2\sumo jm \sumo km (\ol g(j)-\ol g(k))^2 w_j \fc{w_k}{\chi^2(p_j||p_k)}\\
&\le \rc2\sumo jm \sumo km \Var_{p_j}(g)w_jw_k &\text{by Lemma~\ref{lem:change-dist}}\\
&\le 
\rc2\sumo jm w_j C\sE_j(g,g) = 
\fc C2 \sE(g,g).
\end{align}
Thus
\begin{align}
\eqref{eq:to-cont}
%&\le C \sE(g,g) + \ol C \Var_{p}(g)\\
&\le C \sE(g,g) + \fc{\ol C C}2\sE (g, g)
\end{align}
as needed.
\end{proof}

==> gap2.tex <==

\subsection{$\chi^2$ Gap-Product Theorem for Simulated Tempering}


\begin{thm}[$\chi^2$ Gap-Product Theorem for Simulated Tempering]
\label{thm:gap-prod-st}
Consider simulated tempering $M$ with Markov chains $M_i=(\Om,\sL_i)$, $1\le i\le L$. Let the stationary distribution of $M_i$ be $p_i$, the relative probabilities be $r_i$, and the rate be $\la$. Let the Dirichlet form be $\sE_i(g,h) = -\an{g,\sL_i h}$.

Represent a function $g\in  [L]\times \Om$ as $(g_1,\ldots, g_L)$. Let $p$ be the stationary distribution on $[L]\times \Om$, $\sL$ be the generator, and $\sE(g,h) = -\an{g,\sL h}$ be the Dirichlet form.
%, and write $p=\sumo iL r_i p_i$ by thinking of $p_i$ as a distribution on $\Om\times \{i\}$.

Suppose the following hold.
\begin{enumerate}
\item
There is a decomposition
\begin{align}
p_i \sL_i &=\sumo j{m_i} w_{i,j}p_{i,j} \sL_{ij}\\
%\an{g_i, \sL_ig_i}_{p_i} &= \sum_{j=1}^{m_i} w_{i,j} \an{g_i, \sL_{ij}g_i}_{p_{i,j}}\\
p_i &= \sumo j{m_i} w_{i,j}p_{i,j}.\label{eq:decomp}
\end{align}
where $\sL_{ij}$ is the generator for some Markov chain $M_{i,j}$ on $ \{i\}\times\Om$ with stationary distribution $p_{i,j}$.
\item
(Mixing for each $M_{i,j}$) $M_{i,j}$ satisfies the Poincar\'e inequality
\begin{align}
\Var_{p_{i,j}}(g) &\le C \sE_{i,j}(g,g).
\end{align}
\item
(Mixing for projected chain) 
Define the $\chi^2$-projected chain $\ol M$ as the Markov chain on $[n]$ generated by $\ol{\sL}$, where $\ol{\sL}$ acts on $\ol g\in L^2([n])$ by
\begin{align}
\ol{\sL} \ol g(i,j) &= 
\sumo iL \sumo j{m_i} 
\sumo {i'}L \sumo {j'}{m_{i'}}
[\ol g(i',j') - \ol g(i,j)] \ol P((i,j),(i',j'))\\
\text{where }
\ol{P}((i,j),(i',j'))
&=\begin{cases}
\fc{w_{i,j'}}{\max\{\chi^2(p_{i,j}||p_{i,j'}), \chi^2(p_{i,j'}||p_{i,j})\}}
,&i=i'\\
\fc{\min\bc{\fc{r_{i'}w_{i',j'}}{r_i w_{i,j}},1}}{\max\{\chi^2(p_{i,j}||p_{i',j'}), \chi^2(p_{i',j'}||p_{i,j})\}}
,&i'=i\pm 1\\
0,&\text{else.}
\end{cases}\label{eq:chi-trans-p}
\end{align}
Let $\ol p$ be the stationary distribution of $\ol M$. 
Then $\ol M$ satisfies the Poincar\'e inequality
\begin{align}
\Var_{\ol p} (\ol g) & \le \ol C \ol{\sE}(g,g).
\end{align}
\end{enumerate}
Then $M$ satisfies the Poincar\'e inequality
\begin{align}
\Var(g) &\le \max\bc{C \pa{1+\fc{13}{2}\ol C}, \fc{6\ol C}{\la}} \sE(g,g).
\end{align}
\end{thm}
The proof starts as before. The new part is that the projected Markov chain involves transitions between levels, so $\ol{\sE}$ will involve taking differences of functions on adjacent levels. That part will be bounded by the second term in~\eqref{eq:dir-st}.
\begin{proof}
First, note that the stationary distribution $\ol p$ of $\ol M$ is given by $\ol p((i,j)) = r_i w_{i,j}$, because $\ol P((i,j),(i',j')) r_iw_{i,j} = \ol P((i',j'), (i,j)) r_{i'}w_{i',j'}$. 

Given $g\in L^2([L]\times \Om)$, define $\ol g\in L^2\pa{\bigcup_{i=1}^L( \{i\}\times [m_i])}$ by $\ol g(i,j) = \EE_{p_{i,j}} g_i$.
\begin{align}
\Var_p(g) &=\sumo iL \sumo j{m_i} r_{i}w_{i,j} \int (g-\EE_p g)^2p_j\\
&=\sumo iL \sumo j{m_i} r_{i}w_{i,j}
\ba{
\pa{\int (g_i-\EE_{p_{i,j}} g_i)^2 p_{i,j}}
+(\EE_{p_{i,j}} g_i - \EE_p g)^2}\\
&\le C \sumo iL \sumo j{m_i} r_{i}w_{i,j} \sE_{{i,j}}(g_i,g_i) + \Var_{\ol p}(\ol g)\\
&\le C \sumo iL r_i \sE_i(g_i,g_i) + \ol C \ol \sE (\ol g, \ol g).
\label{eq:to-cont2}
\end{align}
Now $\ol{\sE}$ has two terms; the first is bounded in the same way as the Theorem~\ref{thm:gap-prod}.
\begin{align}
\ol \sE(\ol g, \ol g) &=\rc2\ub{ \sumo iL \sumo jn \sumo{j'}n (\ol g(i,j)-\ol g(i,j'))^2
r_iw_{i,j}\ol P((i,j),(i,j'))}{A} \\
&\quad + 
\rc 2\ub{\sumo iL
\sumo j{m_i}
\sumr{i'=i\pm 1}{1\le i'\le L}
\sumo j{m_{i'}}
 (\ol g(i,j)-\ol g(i',j'))^2
r_iw_{i,j}\ol P((i,j),(i',j'))}{B}\\
%\sumo iL \sumo jn \sumo{j'}n (\ol g(i,j)-\ol g(i,j'))^2
%r_iw_{i,j}\ol P((i,j),(i,j'))
A&\le 
\sumo iL \sumo j{m_i} \sumo{j'}n (\ol g(i,j)-\ol g(i,j'))^2
r_iw_{i,j}\fc{w_{i,j'}}{\chi^2(p_{i,j}||p_{i,j'})}\\
&\le \sumo iL \sumo j{m_i}  r_i w_{i,j} \Var_{p_{i,j}}(g_i)&\text{by Lemma~\ref{lem:change-dist}}\\
&\le \sumo iL %\sumo j{m_i}
 r_i C\sE_{i}(g_i,g_i).
\end{align}
For the second term, we use Lemma~\ref{lem:change-dist-f}.
\begin{align}
%\sumo iL
%\sumo j{m_i}
%\sumr{i'=i\pm 1}{1\le i'\le L}
%\sumo j{m_{i'}}
% (\ol g(i,j)-\ol g(i',j'))^2
%r_iw_{i,j}\ol P((i,j),(i',j'))
B
&\le 
\sumo iL
\sumo j{m_i}
\sumr{i'=i\pm 1}{1\le i'\le L}
\sumo {j'}{m_{i'}}
\ba{
6 \Var_{p_{i,j}}(g_i) \chi^2(p_{i,j}||p_{i',j'}) + 
3  \int_\Om (g_i-g_{i'})^2 \min\{p_{i,j},p_{i',j'}\}
}
%3\ba{
%\Var_{p_{i,j}}(g_i) \chi^2(p_{i,j}||p_{i',j'}) +
%\Var_{p_{i',j'}}(g_{i'}) \chi^2(p_{i',j'}||p_{i,j})
%+ \int (g_i-g_{i'})^2 \min\{p_{i,j},p_{i',j'}\}
%}
r_iw_{i,j}\ol P((i,j),(i',j'))\\
&\le 
\sumo iL
\sumo j{m_i}
\sumr{i'=i\pm 1}{1\le i'\le L}
\sumo {j'}{m_{i'}}
\ba{6 r_iw_{i,j}\Var_{p_{i,j}}(g_i) w_{i',j'}
+ 3 r_iw_{i,j} 
\min\bc{\fc{r_{i'}w_{i',j'}}{r_i w_{i,j}}, 1}
 \int_\Om (g_i-g_{i'})^2 \min\{p_{i,j},p_{i',j'}\}
}\\
&=12
\sumo iL
\sumo j{m_i} r_iw_{i,j}\Var_{p_{i,j}}(g_i)
 + 3\sumo iL
\sumo j{m_i}
\sumr{i'=i\pm 1}{1\le i'\le L}
\sumo j{m_{i'}}
\int_\Om (g_i-g_{i'})^2 \min\{r_iw_{i,j}p_{i,j},r_{i'}w_{i',j'}p_{i',j'}\}\\
&\le 12 \sumo iL r_i C\sE_i(g_i,g_i) + 3
%\fc{6}{\la} \fc{\la}2 
\sumo iL \sumr{1\le i'\le m}{i'=i\pm 1}\int_\Om (g_i-g_{i'})^2 \min \{r_ip_i,r_{i'}p_{i'}\}
\end{align}
Then 
\begin{align}
\eqref{eq:to-cont2}
&\le C\sumo iL r_i \sE_i(g_i,g_i)
+\fc{\ol C}2
\pa{
13 C\sumo iL r_i \sE_{i}(g_i,g_i) + 
\fc{12}{\la} \fc{\la}2 
\sumo iL \sumr{1\le i'\le L}{i'=i\pm 1} (g_i-g_{i'})^2 \min \{r_ip_i,r_{i'}p_{i'}\}
}\\
&\le 
\max\bc{C \pa{1+\fc{13}2\ol C}, \fc{6\ol C}{\la}}
\sE(g,g).
\end{align}
\end{proof}
